Language Embeddings for Typology and Cross-lingual Transfer Learning

Cross-lingual language tasks typically require a substantial amount of annotated data or parallel translation data. We explore whether language representations that capture relationships among languages can be learned and subsequently leveraged in cross-lingual tasks without the use of parallel data. We generate dense embeddings for 29 languages using a denoising autoencoder, and evaluate the embeddings using the World Atlas of Language Structures (WALS) and two extrinsic tasks in a zero-shot setting: cross-lingual dependency parsing and cross-lingual natural language inference.

==> ethics.tex <==
\section*{Ethical Consideration}
Our motivation to learn language embeddings without parallel data is to understand how language relationships and typology can be generated without any human annotation. 
We also explore how our learned language embeddings can be applied to downstream tasks. We hope that our proposed method can inspire future research on generating and utilizing typology in cross-lingual settings because we may not have a large amount of translation data for each language, which has been widely  used in past research on data-driven  modeling of linguistic typology. Since our proposed method can be easily adapted to different architectures and pre-trained models with minimal cost (in terms of both data annotation cost and computation cost), it can reduce resources needed when applying language embeddings for zero-shot cross-lingual downstream tasks. We run all our experiments on two TITAN RTX GPUs and two RTX 2080Ti GPUs. We compare our language embeddings to baselines in the standard settings in literature.


==> results_tables/WALS_results.tex <==
\begin{table}[h]
% \small
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cccc|c}
\toprule

& Lexicon & Syntax & Part. Morph. & Non-learn. & Rand \\

$n$ features & 2 & 14 & 46 & 20 & - \\
\midrule
Random  & 0.56 & 0.61 & 0.52 & 0.52 & -  \\
Majority  & 0.64 & 0.75 & 0.69 & 0.68 & - \\
\midrule
Malaviya & 0.66\sig & 0.74 & 0.66 & 0.66 & 0.13\\
XLM mono & 0.41 & 0.75 & 0.66 & 0.68 & 0.12\\
\midrule
Spe. & 0.64 & 0.78\sig & 0.68 & 0.66 & 0.53\\
Eng. & 0.85\sig & 0.79\sig & \textbf{0.71\sig} & 0.66 & \textbf{0.58}\\
Wiki & \textbf{0.87\sig} & \textbf{0.81\sig} & 0.70\sig & \textbf{0.68} & 0.51\\

\bottomrule
\end{tabular}
}
\end{center}

\caption{\label{wals_results} WALS prediction and linguistic typology clustering results on 26 in-common languages across 10 language genera. 
% WALS features are grouped into categories, and the table shows the average accuracy (\%) in each category.
\sig indicates statistical significance ($p<0.01$) over the Majority baseline.}
% Significantly above the Majority baseline ($p<0.01$, single-tail T test)
\end{table}



==> results_tables/XNLI_results.tex <==
\begin{table*}[t]
\small
\begin{center}
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccccc|c}
\toprule
% \hline
& fr             & es    & de    & el    & bg    & ru    & tr    & ar    & vi  & avg.  \\ 
\midrule
\multicolumn{11}{l}{\textit{Selected with English development set}}     \\
\midrule
XLM & 77.3 & 77.9 & 75.9 & 74.3 & 75.3 & 73.8 & 70.4 & 70.9 & 73.2 & 74.3 \\ 
XLM + lang\_emb & \textbf{78.3} & \textbf{79.0} & \textbf{76.5} & \textbf{75.6} & \textbf{76.6} & \textbf{74.8} & \textbf{71.3} & \textbf{72.3} & \textbf{74.4} & \textbf{75.4} \\
\midrule
\multicolumn{11}{l}{\textit{Selected with averaged development set}}     \\
\midrule
XLM & 77.4 & 78.2 & 76.1 & 75.4 & 76.3 & 74.4 & 70.3 & 71.7 & 73.5 & 74.8 \\ 
XLM + lang\_emb & \textbf{78.5} & \textbf{79.0} & \textbf{76.7} & \textbf{75.9} & \textbf{76.8} & \textbf{75.3} & \textbf{71.5} & \textbf{72.4} & \textbf{74.8} & \textbf{75.7}\\
\midrule
XLM-R\textsubscript{Base}  & 77.9 & 78.7 & 76.9 & 76.0 & 77.9 & 75.9 & 72.4 & 72.2 & 74.8 & 75.9 \\
XLM-R\textsubscript{Base} + lang\_emb & \textbf{78.8} & \textbf{79.4} & \textbf{77.4} & \textbf{76.2} & \textbf{78.2} & \textbf{76.1} & \textbf{73.2} & \textbf{72.6} & \textbf{75.4} & \textbf{76.4} \\
\midrule
XLM-R\textsubscript{Large}  & 83.6 & 84.6 & 83.0 & 82.4 & 83.3 & 80.3 & 79.1 & 79.0 & 80.0 & 81.7 \\
XLM-R\textsubscript{Large} + lang\_emb & \textbf{83.9} & \textbf{84.8} & \textbf{83.7} & \textbf{82.8} & \textbf{84.2} & \textbf{81.1} & \textbf{80.3} & \textbf{79.4} & \textbf{80.3} & \textbf{82.3} \\

\bottomrule
\end{tabular}
}
\end{center}
\caption{\label{xnli_results_MUSE} Results on XNLI test set with zero-shot prediction. The results show that adding language embeddings outperforms the baselines in all settings.}
\end{table*}

==> results_tables/app_den_par.tex <==
\begin{table}[h!]
\small
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
\toprule
Language & Spe. & Wiki & XLM mono \\
\midrule
\multicolumn{3}{l}{\textit{Finnic}} \\
\quad Estonian & 60.27 & 61.36 & 53.51\\
\quad Finnish & 62.49 & 62.32 & 55.65 \\
%midrule
\multicolumn{3}{l}{\textit{Germanic}} \\
\quad Danish & 68.81 & 70.37 & 66.48 \\
\quad English & 73.00 & 69.68 & 70.96 \\
\quad German & 63.64 & 65.49 & 64.01\\
\quad Norwegian & 77.76 & 75.42 & 74.24 \\
\quad Slovene & 71.17 & 71.19 & 64.29 \\
%\midrule
\multicolumn{3}{l}{\textit{Romance}} \\
\quad Catalan & 81.72 & 81.95 & 79.13\\
\quad French & 78.57 & 79.27 & 72.52 \\
\quad Spanish & 83.38 & 82.09 & 81.40\\
\quad Portuguese & 79.65 & 80.09 & 80.40 \\
%\midrule
\multicolumn{3}{l}{\textit{Semitic}} \\
\quad Arabic & 52.58 & 51.26 &  50.58\\
\quad Hebrew & 38.93 & 33.01 & 47.56 \\
%\midrule
\multicolumn{3}{l}{\textit{Slavic}} \\
\quad Bulgarian & 66.22 & 64.57 & 62.09\\
\quad Czech & 67.31 & 59.15 & 64.66\\
\quad Russian & 62.92 & 62.08 & 62.04 \\
\midrule
Average & 68.02 & 66.83 &  65.60\\
\bottomrule
\end{tabular}
% }
\caption{\label{app_dependency_results} Zero-shot parsing results (UAS) comparing Spe., Wiki, and XLM mono language embeddings. Results show that using language embeddings can improve parsing performance, and our methods outperform previous methods by a large margin (2.4 absolute points).}
\end{table}

==> results_tables/app_xlmr.tex <==
\begin{table*}[h]
\small
\begin{center}
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccccc|c}
\toprule
% \hline
& fr             & es    & de    & el    & bg    & ru    & tr    & ar    & vi  & avg.  \\ 
\midrule
\multicolumn{11}{l}{\textit{Selected with averaged development set}}     \\
\midrule
XLM-R\textsubscript{Base} + Spe. & 78.9 & 79.8 & 77.2 & 76.0 & 78.2 & 76.2 & 73.8 & 72.5 & 75.3 & 76.4 \\
\midrule
XLM-R\textsubscript{Base} + Wiki & 79.0 & 78.7 & 76.4 & 76.1 & 78.3 & 75.9 & 73.8 & 71.8 & 75.5 & 76.2 \\
\midrule
XLM-R\textsubscript{Base} + XLM mono & 78.2 & 78.4 & 76.7 & 76.4 & 78.1 & 75.9 & 73.6 & 72.3 & 75.1 & 76.1 \\
\midrule
XLM-R\textsubscript{Base} + XLM parallel & 78.3 & 78.9 & 76.5 & 76.6 & 77.6 & 75.4 & 73.2 & 72.4 & 75.0 & 76.0 \\

\bottomrule
\end{tabular}
}
\end{center}
\caption{\label{app_xnli_results} Results on XNLI test set with zero-shot prediction comparing different language embeddings on XLM-R\textsubscript{Base}. We cannot compare directly to machine translation-based methods such as \citet{malaviya-etal-2017-learning} because there is no English embeddings. The results show that on XLM-R\textsubscript{Base}, our language embeddings perform better than language embeddings from previous research.}
\end{table*}

==> results_tables/dependency_parsing_results.tex <==
\begin{table}[h]
% \small
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
Language & Baseline & Language Emb. \\
\midrule
\multicolumn{3}{l}{\textit{Finnic}} \\
\quad Estonian & 56.19 & \textbf{61.68} \small{(+5.49)}\\
\quad Finnish & 59.59 & \textbf{62.91} \small{(+3.32)}\\
%midrule
\multicolumn{3}{l}{\textit{Germanic}} \\
\quad Danish & 63.31 & \textbf{69.62} \small{(+6.31)}\\
\quad English & \textbf{74.51} & 74.08 \small{(-0.43)}\\
\quad German & 64.36 & \textbf{65.67} \small{(+1.31)}\\
\quad Norwegian & 77.19 & \textbf{78.20} \small{(+1.01)}\\
\quad Slovene & 67.92 & 67.91 \small{(-0.01)}\\
%\midrule
\multicolumn{3}{l}{\textit{Romance}} \\
\quad Catalan & 72.41 & \textbf{80.76} \small{(+8.35)}\\
\quad French & 68.75 & \textbf{79.37} \small{(+10.62)}\\
\quad Spanish & 74.42 & \textbf{81.74} \small{(+7.32)}\\
\quad Portuguese & 71.11 & \textbf{79.57} \small{(+8.46)}\\
%\midrule
\multicolumn{3}{l}{\textit{Semitic}} \\
\quad Arabic & 48.44 & \textbf{52.51} \small{(+4.07)} \\
\quad Hebrew & \textbf{41.87} & 33.66 \small{(-8.21)}\\
%\midrule
\multicolumn{3}{l}{\textit{Slavic}} \\
\quad Bulgarian & 62.91 &\textbf{ 67.00} \small{(+1.09)}\\
\quad Czech & 65.62 & \textbf{66.98} \small{(+1.36)}\\
\quad Russian & 62.10 & \textbf{66.45} \small{(+4.35)}\\
\midrule
Average & 64.61 & \textbf{68.01} \small{(+3.40)} \\
\bottomrule
\end{tabular}
}
\caption{\label{tab:dependency_results} Zero-shot parsing results (UAS), where
each of 16 languages are parsed using annotated language from the other
15 languages. In the \textit{Language Emb.} column, results were obtained by
concatenating the language embedding to each token's MUSE embedding. In the 
\textit{Baseline} column, results were obtained using a random embedding
instead. Boldface indicates a statistically significant difference ($p<0.05$).}
\end{table}

==> results_tables/word_translation.tex <==
\begin{table*}[h]
\small
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccccccc}
\toprule
& en     & fr    & es    & de    & el    & bg    & ru    & tr   & he   & ar    & vi   \\
\midrule
en & 100.00 & 83.00 & 83.85 & 77.07 & 59.81 & 60.86 & 67.51 & 61.48 & 58.69  & 52.04 & 54.57 \\
\bottomrule
\end{tabular}
}
\caption{Precision at k = 1 word translation to English for the most frequent 50,000 words in each language using CSLS for the generated dictionary.} \label{word_translation_accuracy}
\end{center}
\end{table*}

